Unique Solutions of Guarded Recursive Equations

This paper shows that guarded systems of recursive equations have unique solutions up to strong bisimilarity for any process algebra with a structural operation semantics in the ready simulation format. A similar result holds for simulation equivalence, for ready simulation equivalence and for the (ready) simulation preorder. As a consequence, these equivalences and preorders are full (pre)congruences for guarded recursion. Moreover, the unique-solutions result yields a sound and ground-complete axiomatisation of strong bisimilarity for any finitary GSOS language.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{C. Di Giusto and G. Bacci (Eds.): Combined \\
Workshop on Expressiveness in Concurrency and \\
Structural Operational Semantics (EXPRESS/SOS 2025)\\
EPTCS 433, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.433.6}{10.4204/EPTCS.433.6}}
\pdfoutput=1

